This Reads Like That: Deep Learning for Interpretable Natural Language Processing

Prototype learning, a popular machine learning method designed for inherently interpretable decisions, leverages similarities to learned prototypes for classifying new data. While it is mainly applied in computer vision, in this work, we build upon prior research and further explore the extension of prototypical networks to natural language processing. We introduce a learned weighted similarity measure that enhances the similarity computation by focusing on informative dimensions of pre-trained sentence embeddings. Additionally, we propose a post-hoc explainability mechanism that extracts prediction-relevant words from both the prototype and input sentences. Finally, we empirically demonstrate that our proposed method not only improves predictive performance on the AG News and RT Polarity datasets over a previous prototype-based approach, but also improves the faithfulness of explanations compared to rationale-based recurrent convolutions.

==> parts/discussion.tex <==
\section{Discussion}
In this section, we discuss our obtained results.

\subsection{Weighted Similarity Measure}
For all our experiments, we demonstrate that the model seems to learn from the right sentence embedding dimensions such that over all experiments the accuracy improved (cf. Table \ref{tab:weighted_experiments}). The largest change can be observed when using standard cosine similarity on the AG news dataset with an accuracy of 78.86\% going up by almost 8\%-points to an accuracy of 86.38\% when using learned embedding dimensions weighing inside the cosine similarity metric. We observe, that for both datasets, the standard as well as the learned weighted cosine similarity performed better than $\ell_2$ or learned weighted $\ell_2$ similarity.


\subsection{Ablation Studies of Losses}
In general, we observe that for the baseline model with all loss terms included, the model largely relies on the top 2 prototypes, as without them accuracy drops to 27.89\%. 

The clustering loss, $\text{Clst}(\mathbf{z}, \mathbf{p}): \mathbb{R}^d \times \mathbb{R}^d \longrightarrow \mathbb{R}$, should ensure that each training sample is close to at least one prototype whereas the separation loss, $\text{Sep}(\mathbf{z}, \mathbf{p}): \mathbb{R}^d \times \mathbb{R}^d \longrightarrow \mathbb{R}$, should encourage training samples to stay away from prototypes not of their own class \cite{li2018deep}. In the results, we can see that seemingly the full loss ($\lambda_i \neq 0, i \in \{1,...,5\}$) relies more on the top 2 prototypes, as accuracy is much lower for the model with the clustering term removed than for the model with the full loss term. This suggests that without this term the model may rely on many prototypes to get to an estimate instead of only on the most similar prototype as it should encourage. 

Results after removing the separation loss term show a slightly higher accuracy of 83.37\% and a stronger drop-off when removing the prototypes. The steeper drop-off may imply that it has the desired effect of separating prototypes of different classes appropriately. 

The goal of the distribution loss, $\text{Dist}(\mathbf{z}, \mathbf{p}): \mathbb{R}^d \times \mathbb{R}^d \longrightarrow \mathbb{R}$, is to ensure that each prototype is close to a sample in the training set. The removal of this loss does not seem to hurt the performance. Hence, we believe it is not necessary and could be removed. A possible explanation of this behaviour might be that while theoretically the maximum is specified over the whole training set, in the code of \citet{protonlp} that we adopted, the maximum is only taken over a batch. Requiring each prototype to be close to a training sample from each batch might be too much to ask for. Further research might be going into a relaxation of this loss. 

The idea of the diversity loss, $\text{Divers}(\mathbf{p}): \mathbb{R}^d \longrightarrow \mathbb{R}$, is to push prototypes from the same class apart to learn different facets of the same class \cite{protonlp}. Compared to the baseline, the results show that indeed accuracy is higher when removing the top $k$ prototypes and the diversity loss term seems to have the desired effect of prototypes learning different facets of the same class. 

Finally, dropping the weights' $\ell_1$-regularization term does seem to slightly worsen the performance when dropping 1 to 3 prototypes.

If paper: Change this to another title as we're not only talking about Protovis
\subsection{Prototype Visualization}
Thanks to our innovation, we go beyond simply visualizing the prototypical sentence and show the most important words from the prototype as well as from the sample we are comparing it to. This way, we enhance the interpretability mechanism, as we can show to which words from the prototype, the test sample is most similar to and which words from it actually contributed most to the similarity. Overall though, this means that the most important words from the same prototype can actually differ depending on the test sample.

\subsection{Faithfulness}
In terms of accuracy, between the baseline model \cite{lei2016rationalizing} and ours there already exist an 4\%-points improvement. Note that the accuracy is not comparable to Table~\ref{tab:weighted_experiments} as the dataset differs. Looking at the interpretability metrics, the results suggest that our model is more \textit{faithful}. Our model, with a sufficency value of -0.2316, has a lower score than the baseline model with -0.1348, indicating that the rationals were more important for the prediction in our model. 
Additionally, the comprehensiveness score of our model is 2\%-points lower than the baseline model, Thus, seemingly our model takes more context (besides the rational) into account when predicting compared to the baseline model. This is also what the baseline model was critiqued for, as it potentially takes Trojan explanations for classification instead of attending mainly to the rational with some context as well (cf. Section \ref{ssec:rational_models}). 
Furthermore, we interpret this as our model using mainly the rationale for prediction, compared to the baseline model. This is also reflected in the accuracy of the rational-only and the accuracy without the rational in both models, since our models' accuracy is much higher for the rational-only and significantly lower for the sample without the rational. 

%Fyi han d acknowledgement section wieder inegnoh will ich denkt han du hesch sie viliccht usversehe usegnoh? Sust chasch sie gern wieder useneh, I don't care.

==> parts/ethics_statement.tex <==
\section*{Ethics Statement}
Scientific work published at EMNLP 2023 must comply with the \href{https://www.aclweb.org/portal/content/acl-code-ethics}{ACL Ethics Policy}. We encourage all authors to include an explicit ethics statement on the broader impact of the work, or other ethical considerations after the conclusion but before the references. The ethics statement will not count toward the page limit (8 pages for long, 4 pages for short papers).


==> parts/experiments.tex <==
% 1. Weighted similarity metric improves performance
% 2. Loss ablation study using our best model from previous improvements
% 3. Enhanced interpretability
%     3.1 interpretability metrics for faithfulness (comprehensiveness & sufficiency) for our best model & Rational model as baseline
%     3.2 Interpretability mechanism extension from ProtoTrex by allowing to extract keywords from prototype and test sample
\section{Experiments}
In this section, we present the experiments we conducted to show the importance of the methods we proposed in the previous section.
\subsection{Learned Weighted Similarity Metric}
To explore the impact of the weighted embedding dimensions in the similarity metric, we carry out an experiment where we compare the weighted with the unweighted performance on the movie review dataset~\cite{moviereview_ds} as well as the AG news dataset~\cite{news_ds}.

Table~\ref{tab:weighted_experiments} shows the accuracy results from the experiments using the learned weighted similarity metrics. 


\begin{table}[!h]
\centering
\begin{tabularx}{\columnwidth}{@{}lrr@{}}\toprule % removing whitespace on the right does not seem to work
& \multicolumn{2}{c@{}}{Dataset} \\
\cmidrule{2-3}
\textbf{Similarity metric}    &   \textbf{RT polarity} &  \textbf{AG news}\\
\midrule
Cosine & 80.02 &  78.59   \\
\gray{\small95\%-CI} & \gray{\small(78.29, 81.70)} & \gray{\small(77.70, 79.47)}   \\
Weighted cosine & \textbf{82.65} & \textbf{86.50}   \\
\gray{\small95\%-CI} & \gray{\small(80.98, 84.33)} & \gray{\small(85.74, 87.29)}   \\
$\ell_2$ distance & 78.29& 75.09    \\
\gray{\small95\%-CI} & \gray{\small(76.61, 80.11)} & \gray{\small(74.13, 76.03)}   \\
Weighted $\ell_2$ distance & \textbf{80.35} & \textbf{78.07}   \\
\gray{\small95\%-CI} & \gray{\small(78.63, 81.98)} & \gray{\small(77.16, 79.03)}   \\
\bottomrule
\end{tabularx}
\caption{Test accuracy results from sentence ProtoTrex \cite{protonlp} using their standard similarity metrics and our learned embedding dimensions' weighted similarity metrics.}
\label{tab:weighted_experiments}
\end{table}


\subsection{Visualizing Important Words}
% What important words in prototypes in NLP look like
% How good are the results (metrics) with prototypes (showing results without them)
% Interpretability of prototype network in NLP
To demonstrate the effectiveness of our approach, we show qualitative samples from the test set of the movie review. Table \ref{tab:samples} presents test set sentences with prototypes and the corresponding most important words from the sentence itself but also from the prototype. 

\begin{table*}[]
\centering
\begin{tabularx}{\textwidth}{@{}XX@{}}
\toprule
\textbf{Sample and its keywords} & \textbf{Prototype 1 and its most important words}\\
\midrule
$\bullet$ This \hl{insufferable} \hl{movie} is meant to make you think about existential suffering. Instead, it'll \hl{only} put you to \hl{sleep}. &$\bullet$ Plodding, \hl{poorly} written, murky and weakly \hl{acted}, the picture feels as if \hl{everyone} making it \hl{lost} their \hl{movie} mojo. \\ 
$\bullet$ Because of an \hl{unnecessary} and \hl{clumsy} last scene,' swimfan' left me with \hl{a} very \hl{bad} feeling. &$\bullet$ \hl{Plodding}, \hl{poorly} written, murky and \hl{weakly} acted, the picture feels as if everyone making it \hl{lost} their movie mojo.  \\
$\bullet$ Campanella's \hl{competent} direction and his \hl{excellent} cast \hl{overcome} the obstacles of a predictable outcome and a \hl{screenplay} that glosses over \hl{rafael's} evolution. 
&$\bullet$ ...\hl{bright}, \hl{intelligent}, \hl{and} humanly \hl{funny} film. \\
$\bullet$ Between them, de niro and \hl{murphy} make showtime the \hl{most} savory and \hl{hilarious} guilty \hl{pleasure} of many a recent movie season. 
& $\bullet$ ...\hl{bright}, \hl{intelligent}, and humanly \hl{funny} \hl{film.} \\
\bottomrule
\end{tabularx}
\caption{Exemplary test samples from the movie review dataset by \citet{moviereview_ds} with the corresponding most important prototype from training. The most important words as determined by our model are visualized in \hl{color}.}
\label{tab:samples}
\end{table*}

% \begin{table*}[!h]
% \centering
% \begin{tabularx}{\textwidth}{@{}XX@{}}
% \toprule
% \textbf{Sample and its keywords} & \textbf{Prototype 1 and its most important words}\\
% \midrule
% This \hl{insufferable} \hl{movie} is meant to make you think about existential suffering. Instead, it'll \hl{only} put you to \hl{sleep}. & Plodding, \hl{poorly} written, murky and weakly \hl{acted}, the picture feels as if \hl{everyone} making it \hl{lost} their \hl{movie} mojo. \\ 
% Because of an \hl{unnecessary} and \hl{clumsy} last scene,' swimfan' left me with \hl{a} very \hl{bad} feeling. & \hl{Plodding}, \hl{poorly} written, murky and \hl{weakly} acted, the picture feels as if everyone making it \hl{lost} their movie mojo.  \\
% \bottomrule
% \end{tabularx}
% \caption{Exemplary test samples from the movie review dataset by \citet{moviereview_ds} with the corresponding prototype from training and the keywords in both phrases.}
% \label{tab:samples}
% \end{table*}

\subsection{Faithfulness}
To assess the interpretability mechanism of our model we follow \citet{aligning} and \citet{eraser} and compute comprehensiveness, as well as sufficiency, as proxies for the faithfulness of the model. 
We analyse the faithfulness of the model to its predicted rationals by calculating the change in probability of the predicted label, when removing the rationals or when inputting only the rationals. The previous work of \citet{protonlp} struggles with calculating these measures, as they do not extract specific rationals of a test sentence. Hence, they argue that removing a prototype is similar to a rationale. We believe these two things are vastly different.

Thanks to our improvement outlined in Section~\ref{Visualization}, our method can extract rationals from a test sentence. Therefore, in contrast to \citet{protonlp}, we can truthfully calculate the faithfulness measures.

However, due to the computational complexity of having to compute the rationals for each test sample, we refrain from doing this and leave this to future work with more computing power at hand. Instead, we use human-annotated rationals for the true class as proxies for our predictions to analyse how faithfully the model relies on these important sentence parts. Hence, we show the faithfulness of our model by computing comprehensiveness and sufficiency on the movie review dataset with human-annotated rationals by \citet{eraser}. Table \ref{tab:comp_suff} shows the obtained results. 

Sufficiency is computed as the difference of probability of the predicted class of the unaltered input and the probability of the same class when predicting only using the rationales. It captures the degree to which the extracted rationales are adequate for a model to make a prediction \cite{eraser}.

Comprehensiveness is equivalently calculated, but rather than removing only the rationales, the predicted probability without any rationales is subtracted. A higher score in comprehensiveness implies that the rationals influenced the prediction as is desired.

\begin{table*}[b]
\centering
\begin{tabularx}{\textwidth}{@{}Xrrrrr@{}}\toprule % removing whitespace on the right does not seem to work
\textbf{Model}    & \textbf{Comp. $\uparrow$} &  \textbf{Suff. $\downarrow$} & \textbf{Accuracy (\%)}\\
\midrule
Rationals \cite{lei2016rationalizing} & 0.1505 & 0.0079 &  73.79  \\
\gray{\small 95\%-CI} & \gray{\small(0.3368, 0.3495)} &\gray{\small(-0.0023, 0.0140)} & \gray{\small(71.87, 75.75)} \\ 
Weighted Cosine ProtoTrex & 0.5290  & 0.0263 & 82.65 \\
\gray{\small 95\%-CI} & \gray{\small(0.5179, 0.5412)} &\gray{\small(0.0163, 0.0354)} & \gray{\small(80.98, 84.33)} \\
\bottomrule
\end{tabularx}
\caption{Comprehensiveness (Comp.) and Sufficiency (Suff.) results running our best model and the baseline on the movie review dataset with human annotated rationals \cite{eraser}.}% Change citation here
\label{tab:comp_suff}
\end{table*}


% \subsection{Evaluation}
% \begin{table}[h]
%     \centering
%     \captionsetup{justification=centering}
%     \caption{Example Results Table.}
%     \begin{tabular}{||c|c|c|c||} 
%          \hline
%          \textbf{Test set} & \textbf{Attack} & \textbf{$\epsilon$} & \textbf{Iterations} \\ [0.5ex]
%          \hline \hline
%          adv1 & FGSM & 0.01 & 1\\
%          adv2 & PGD & 0.05 & 20\\
%          adv3 & PGD & 0.01 & 20\\ [0.5ex]
%          \hline
%     \end{tabular}
%     \label{table:attacks}
% \end{table}


